Deep Appearance Prefiltering

Physically based rendering of complex scenes can be prohibitively costly with a potentially unbounded and uneven distribution of complexity across the rendered image. The goal of an ideal level of detail (LoD) method is to make rendering costs independent of the 3D scene complexity, while preserving the appearance of the scene. However, current prefiltering LoD methods are limited in the appearances they can support due to their reliance of approximate models and other heuristics. We propose the first comprehensive multi-scale LoD framework for prefiltering 3D environments with complex geometry and materials (e.g., the Disney BRDF), while maintaining the appearance with respect to the ray-traced reference. Using a multi-scale hierarchy of the scene, we perform a data-driven prefiltering step to obtain an appearance phase function and directional coverage mask at each scale. At the heart of our approach is a novel neural representation that encodes this information into a compact latent form that is easy to decode inside a physically based renderer. Once a scene is baked out, our method requires no original geometry, materials, or textures at render time. We demonstrate that our approach compares favorably to state-of-the-art prefiltering methods and achieves considerable savings in memory for complex scenes.

==> 3_problem_setting_surface.tex <==
\section{Prefiltered Light Transport}
\label{sec:TheoreticalOverview}

\begin{figure}[t]
	\centering
	% \includegraphics[width=\linewidth]{Figures/Framework/LightSamplingHemispheres}
	% \begin{tikzpicture}
	% \def\h{0.24\textwidth}
	% \draw[line width=0.75mm,gray] (0,0.05) -- (0,\h - 0.05);
	% \end{tikzpicture}
	\includegraphics[width=\linewidth]{Figures/Framework/Buildings.png}
	\includegraphics[width=\linewidth]{Figures/Framework/theoretical_overview.pdf}
	
% 	\vspace{-6mm}
	\caption{\Steve{Placeholder image, valid caption.} Here we illustrate how a beam interacts with both large watertight surfaces (buildings) and complex micro-geometry (small tree leaves) as it bounces through the city. The beam begins at the sensor, matching the size of the pixel, and grows with distance based on the parameters of the perspective camera, determining the bandwidth of radiance that gets propagated along its path.} 
	\label{fig:TheoreticalOverview}
	% \vspace{-3mm}
\end{figure}

% \Steve{
% \begin{itemize}
% 	\item As per our discussion on 1/10, this section will introduce the general functions related to our method (e.g., phase function).
% 	\item The next section will then describe how we explicitly represent them
% 	\item A LUT is the naive solution that has problems
% 	\item Our proposed network-based approach can compress, denoise, and interpolate making it a much more practical solution
% 	\item We also need to point out interpolating across scales as part of our algorithm. Even if we just do the typical interpolation strategy, it should be made clear.
% \end{itemize}
% }

\Steve{Section 3.2 and 3.3 are WIP.}

\subsection{Prefiltered Formulation of Path Tracing}

We begin with the rendering equation~\cite{Kajiya86} and omit the emission term for brevity:

\begin{align}
\label{eq:renderingEq}
\radiance{\pos}{\outDir} = \int_{\hemisphere}{\radiance{\pos}{\inDir} \cosbrdfFunc{\pos}{\outDir}{\inDir}  \intOver{\inDir}},
\end{align}

where $\radiance{\pos}{\outDir}$ is the radiance at a surface point, $\pos$, in the outgoing direction, $\outDir$, that comprises of a response of $\cosbrdf$, a Bidirectional Scattering Distribution Function (BSDF), to the incident radiance at $\pos$, or $\radiance{\pos}{\inDir}$, across the whole visible hemisphere $\hemisphere$. Here the BSDF also contains $^{\perp}$, a geometric pullback of the surface manifold, i.e., a cosine term between the incident direction and the surface normal.

In order to introduce prefiltering in path space as it corresponds to a pixel filter, we follow Belcour et al.'s~\shortcite{Belcour17} formulation and highlight relevant components as they pertain to our algorithm.

Using Eq.~\ref{eq:renderingEq}, we can determine the final flux incident on a sensor's pixel, $\pixFlux$, by integrating the radiance incident on the sensor over the pixel filter, $\pixFilter{0}$, also known as a point spread function:

\begin{align}
    \pixFlux &= \int_{\pixSpatAng} 
            \pixFilter{0}(\pos,\outDir)\radiance{\pos}{\outDir}\intOver{\pos}\intOver{\outDir} \\
            %
            &= \int_{\pixSpatAng}\int_{\hemisphere}{\radiance{\pos}{\inDir} \pixFilter{0}(\pos,\outDir)\cosbrdfFunc{\pos}{\outDir}{\inDir}  \intOver{\pos}\intOver{\outDir}\intOver{\inDir}} \\
            %
            &\approx \int{\int{\radiance{\pos}{\inDir} \phaseFunc{0}{\pos}{\outDir}{\inDir} \intOver{\pos}\intOver{\inDir}}}.
\end{align}

Here $\pixSpatAng$ is the pixel footprint, i.e., a spatio-angular integration domain of the pixel filter, comprising all directions through the pixel and all image locations over the pixel area parameterized on the surface. The second line of the equation comes from substituting Eq.~\ref{eq:renderingEq} and rearranging some terms.

In the spirit of Belcour et al.~\shortcite{Belcour17}, for the last line, we also assume the incident radiance, $\radiance{\pos}{\inDir}$, does not change across the pixel footprint (hence the change to $\approx$). This allows us to bring the outer integral inside and integrate over the pixel footprint, replacing the inner product $\langle \pixFilter{0} \cdot \cosbrdf\rangle$ as a \emph{prefiltered phase function}, $\phase{0}$, which determines the throughput of the macro-region covered by the pixel footprint, $\mathcal{F}$.

Again following Belcour et al.~\shortcite{Belcour17} (Eq. 4 in their paper), we can propagate the pixel's footprint to get the prefiltered phase at the $k$th bounce and position, $\newPos$, using

\begin{align}
    \phaseFunc{k}{\newPos}{\outDir}{\inDir} = \int \phaseFunc{k-1}{\pos}{\outDir}{\outDir} \cosbrdfFunc{\pos}{\outDir}{\inDir}  \intOver{\pos}\intOver{\outDir}.
\end{align}

To determine the directional flux at the $k$th bounce, we have

\begin{align}
\fluxFunc{k}{\newPos}{\outDir} = \int{\radiance{\pos}{\inDir}  \phaseFunc{k}{\pos}{\outDir}{\inDir}\cosbrdfFunc{\pos}{\outDir}{\inDir}  \intOver{\pos}\intOver{\inDir}}
\end{align}

% \pixFlux = \sum_{k=0}^{\infty}\int_{\hemisphere}{c\radianceInt{\inDir} \phaseFunc{k}{\pos}{\outDir}{\inDir} \intOver{\pos}\intOver{\inDir}}

This idea is illustrated in Fig.~\ref{fig:TheoreticalOverview}.



% Once we have have a pixel filter propagated towards $k$th bounce, we can integrate the radiance coming from this bounce as
% \begin{align}
%     I^k(\x,\wo) = \int w^k(\x,\wo) \rho(\x,\wo,\wi) L(\x, \wi) \d\wi,
% \end{align}
% where $I^k$ is the directional flux coming from the $k$th bounce, $\rho$ is the phase function prefiltered across the pixel footprint region.


\Steve{This is the original version for reference.}

We start with rendering equation~\cite{Kajiya86} with no emission for brevity:

\begin{align}
\label{eq:re}
  L(\wo) = \int_{\mathcal{H}(\n)}{L(\wi) f_r^{\perp}(\wi,\wo) \, \d \wi},
\end{align}
where $L(\wo)$ is the outgoing radiance at a surface point, that comprises of a response of $f_r^{\perp}$, a Bidirectional Scattering Distribution Function (BSDF) to the incident radiance $L(\wi)$ across the whole visible hemisphere $\mathcal{H}(\n)$ of surface around its normal $\n$. Here the BSDF $f_r$ also contains $^{\perp}$, a geometric pullback of the surface manifold, i.e., a cosine term between the incident direction and the surface normal.

In order to introduce the frequency-based prefiltering, we follow Belcour et al.~\shortcite{Belcour17} and plug Eq.~\ref{eq:re} into the final flux incident on a sensor's pixel. 
% Note, the following derivation follows closely with Belcour et al.'s~\shortcite{Belcour17} and claim no contribution with this regard. We extract the relevant portions as needed to explain our algorithm. 

We need to integrate the radiance incident on the sensor over the pixel filter $w^0$, also known as a point spread function
\begin{align}
    I &= \int_{\mathcal{F}} \!\!\!\!
            w^0(\x,\wo)L(\x,\wo)\d \x \d \wo = 
        %
        \int_{\mathcal{F}}\!\!\!\!
            w^0(\x,\wo)\int_{\mathcal{H}(\n)}\!\!\!\! {L(\wi) f_r^{\perp}(\wi,\wo) \d \wi} \d \x \d \wo \\
        &\approx
            \int_{\mathcal{H}(\n)}\!\!\!\! L(\wi)
            \int_{\mathcal{F}}\!\!\!\!w^0(\x,\wo) f_r^{\perp}(\wi,\wo) \d \x \d \wo \d \wi = \int_{\mathcal{S}}\!\!\!\! L(\wi)
            \rho(\wi) \d \wi,
\end{align}

\Steve{This last line does not seem correct to me. S is the spatial footprint of the pixel filter. Don't we need a double integral to also include dwi (integration over all incident directions)?}
where $\mathcal{F}=\mathcal{A}\times\mathcal{S}$ is the pixel footprint, i.e., a spatio-angular integration domain of the pixel filter, comprising all directions through the pixel and all image locations over the pixel area. 

In the last line, in spirit of Belcour et al.~\shortcite{Belcour17}, we also assume the incident radiance $L(\wi)$ does not change across the pixel footprint and is the reason for the $\approx$. After changing the integration order, we denote the inner product $\langle w \cdot f_r^{\perp}\rangle$ as a \emph{prefiltered phase function} $\rho$ of a region that contains the response of the macroregion covered by the pixel footprint $\mathcal{F}$.

% \Steve{Fig.~\ref{fig:TheoreticalOverview}}

Similarly to Belcour et al.~\shortcite{Belcour17} (Eq. 4 in their paper), we can then extend the footprint propagation to a multi-bounce prefiltered path tracing
\begin{align}
    w^k(\y,\wi) = \int w^{k-1}(\x,\wo)\rho(\x,\wo,\wi)\d\wo,
\end{align}
where $w^k$ is now the pixel filter propagated through $k$ surface interactions.

Once we have have a pixel filter propagated towards $k$th bounce, we can integrate the radiance coming from this bounce as
\begin{align}
    I^k(\x,\wo) = \int w^k(\x,\wo) \rho(\x,\wo,\wi) L(\x, \wi) \d\wi,
\end{align}
where $I^k$ is the directional flux coming from the $k$th bounce, $\rho$ is the phase function prefiltered across the pixel footprint region.

\subsection{Integration along the Filter Beam}

In general scenarios, the assumption of constant incident radiance often breaks because the pixel filter outprojected onto the scene potentially covers multiple disjoint surfaces of the scene. Therefore, the footprint is usually split up into multiple parts along its direction and integrated in parts.

\begin{equation}
   \label{eq:marching}
   \int_A \nabla_{\wo} L (\x, \wo) \d A = I^k(\x,\wo) + \int_A f( L(\x,\wo), \mu(\x,\wo)) \d A
\end{equation}

\psen{One thing I just realized about this equation we came up with is that the $L(\x,\wo)$ in the $f()$ term needs to have something like $\x + \omega \delta t$, because right now the radiance we are talking about is the radiance at the point in question. It needs to be the radiance of a point right behind it. Things makes things a bit messier, though, and I'm not sure what to do about that.}

\psen{Also, we may need to change the domain of integration over the space of angles and points over the footprint of the beam (i.e., your earlier $\mathcal{F}=\mathcal{A}\times\mathcal{S}$), so $\d\omega \d A$ rather than just $\d A$, which would also match Belcour}

\AK{Fig.~\ref{fig:beam}}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{Figures/Framework/beam.pdf}
	%\vspace{-6mm}
	\caption{\Steve{Placeholder image, valid caption.} An illustration of our transmittance model. The beam on the top intersects with the ellipse, rectangle, and quad. On the bottom we show the saturation of the beam's coverage, which determines how much additional radiance can be contributed along the beam. Since it is the first object intersected, the ellipse is unoccluded and its contribution is determined completely by the percent of overlap with the beam. The ellipse and rectangle are anti-correlated (the first blocks the second), so the rectangle has no contribution. Finally, the quad is unobstructed by any of the preceding geometry. It fully saturates the remainder of the beam to full coverage with its contribution, and the beam is terminated. Note, the transmittance tracked on the bottom row shows that such common scenarios are not well approximated by a single model (e.g., linear or exponential), and instead we use a spatial coverage mask within our system to better handle the range of cases.} 
	\label{fig:beam}
	% \vspace{-3mm}
\end{figure}

\subsection{Transmittance}

 \AK{I am not happy with this transition. Ideally, we should be able to reformulate it as a transmittance along the beam.}
%
The final radiance, $\beamRadiance$, accumulated along the beam is given by
\begin{align}
\label{eq:radiance}
L = \sum_{i=0}^{\infty}{\voxWeight_i L(\wi)},
\end{align}
%
where $\voxWeight_i$ and $L(\wi)$ are the weight and incident radiance of the $i$th part, respectively. Note that, $\voxWeight_i \in [0,1]$ and $\sum_{i=0}^{\infty}{\voxWeight_i} = 1$. $L(\wi)$ is computed as discussed in Sec.~\ref{subsec:phaseFunc}, whereas $\voxWeight$ is computed as the difference in beam coverage across the voxel:

%\begin{align}
%\label{eq:voxContribution}
%\voxWeight_i = \beamCoverage_i - \beamCoverage_{i-1}.
%\end{align}

%\subsection{Phase function}
%\label{subsec:phaseFunc}

%General description of phase function goes here.


==> 9_misc.tex <==
\section{Misc}

\Steve{Various junk that I've accumulated (e.g., thoughts, things to explore, deprecated ideas). Items might be deleted or do not have a home currently.}

\Steve{I moved this from Sec.~\ref{subsec:DataGeneration}.} The phase LUT can tell us the RGB throughput for these pair of directions. Then multiplying this by the emitter's radiance value we can find the contribution of that light source to that voxel and ultimately the irradiance at the pixel in the final image by accumulating the contribution from all the voxels.

Once the throughput is calculated, we also compute a 2D coverage mask at each outgoing direction by rendering out an orthographic view of the voxel at a certain resolution (e.g., $128 \times 128$ in our implementation). Each pixel in this coverage map is sampled and if the ray intersects with any geometry in the voxel we record a 1 otherwise we record a 0 for the pixel, thus we have a binary mask that can spatially track the voxel's geometry that is visible in a certain outgoing direction.

To use the coverage mask during rendering, we would track the order of voxels intersected along a beam and accumulate the total beam coverage from voxel to voxel. This accounts for correlation (and anti-correlation) across voxels because we can determine how occluded a voxel is given the voxels before it. In the case the geometry is completely occluded by the previous voxels, then that voxel will have no radiance contribution along the beam. If there was no occlusion at all, then we can add the total throughput. Of course, we can also handle partial coverage similarly by determining an alpha scalar to multiply the throughput by. In the case where multiple voxels are the same distance along a beam, we construct a wavefront and spatially orient the coverage masks to determine the coverage contribution along all those voxels simultaneously. It is also used for calculating the coverage along the shadow beam and subsequent beams during multi-bounce rendering.

Finally, we perform a post-process on the 4D tabular phase function to generate a sampling distribution for selecting the next bounce direction during rendering. Since we only need to choose the next bounce direction based on a given outgoing direction, we only require a 2D PDF using the throughput for the incoming directions. Therefore, we loop through each outgoing direction and normalize the 2D slice containing all of the incoming directions resulting in a 2D table of 2D PDFs. Also, to more efficiently sample these during runtime, we compute the 2D CDFs as well that allow us to find a sample direction from a random number.

% Pre-filtering motivation:
% \begin{itemize}
% 	\item Preserve appearance
% 	\item Reduce rendering costs
% 	\item Enable large compression 
% \end{itemize}

% Background/Motivation for our approach:
% \begin{itemize}
% 	\item Previous work tackled either geometry or material LoD 
% 	\item SotA are hybrid approaches that rely on heuristics with many failure cases and can't handle continuum of in-between cases
% 	\item Propose an ML approach
% \end{itemize}

% \Steve{Previous notes for myself.} Goal is to preserve the appearance of globally lit 3D environments containing complex geometry and materials that are prefiltered for level of detail. To handle a continuum of complex cases and avoid heuristics, we propose to use the first machine learning framework. 

% We choose a multi-scale, voxelized representation of the scene that can be rendered with a beam tracer that combines the voxels in each pixel footprint using their pre-computed phase function and coverage as a 4D lookup table (LUT). Our network learns to compress this LUT into a latent representation (e.g., feature vector) which can then be decoded during runtime to determine the throughput and coverage in a particular pair of incoming/outgoing directions.
\Steve{Other stuff}

Technical challenges:
\begin{itemize}
	\item Network architecture
	\item Training a general network to handle all scenes (need a comprehensive basis training set)
	\item Handling correlation across voxels
\end{itemize}

Overview:
\begin{itemize}
	\item High level framework first describing inference through our pipeline (with an overview figure)
	\item Input and output to the network to illustrate we are baking throughput
\end{itemize}


\subsection{Correlation model}
During data generation, we calculate the local correlation between a voxel and its neighbors, $\correlation_i$, using the coverages from the current voxel, its neighbors, and the combination of the two, $\voxCoverage_{i-1}$, $\voxCoverage_i$, and $\voxCoverage_{i-1,i}$, respectively. Formally, this is written as

\Steve{V is per outgoing direction}

\old{\begin{align}
	\label{eq:correlation}
	\correlation_i = \frac{\voxCoverage_{i-1,i} - [1 - (1 - \voxCoverage_{i-1}) (1 - \voxCoverage_i)]}{(\voxCoverage_{i-1} + \voxCoverage_{i}) - [1 - (1 - \voxCoverage_{i-1}) (1 - \voxCoverage_i)]}.
	\end{align}}

% \begin{align}
% \label{eq:correlation}
% \correlation_i = \frac{\voxCoverage_{i-1,i} - [(1 - \voxCoverage_{i-1}) \voxCoverage_i]}{(\voxCoverage_{i-1} + \voxCoverage_{i}) - [(1 - \voxCoverage_{i-1}) \voxCoverage_i]}.
% \end{align}

\begin{align}
\label{eq:correlation}
\correlation_i = \frac{\voxCoverage_{i-1,i} - \voxCoverage_{i-1} - \voxCoverage_i} {- \voxCoverage_{i-1} \voxCoverage_i}.
\end{align}


During runtime, we can use this correlation factor to compute the beam coverage at the $i$th voxel:

\old{\begin{align}
	\label{eq:beamCoverage}
	\beamCoverage_i ={} & \correlation_i \times (\beamCoverage_{i-1} + \voxCoverage_{i}) \\
	& + (1-\correlation_i) \times [1 - (1 - \beamCoverage_{i-1}) (1 - \voxCoverage_i)].
	\end{align}}

\begin{align}
\label{eq:beamCoverage}
\beamCoverage_i ={} \beamCoverage_{i-1} + \voxCoverage_{i} - \correlation_i \beamCoverage_{i-1} \voxCoverage_{i}
\end{align}


\subsection{Performance considerations}
\Steve{Keep things tractable with strided data generation. What else should go in this section?}

\Steve{Dumping stuff here for now and we can put it where appropriate later.}

Loop through every outgoing direction, which consists of $128^2$ discrete bins separated by a stride of 8 starting from the center bin outwards. Take the u,v at the corner of bin (originally was center of bin) and transform it to cartesian. Set up plane at infinity based on outgoing direction and randomly sample cross section with a uniform distribution. The cross section is the area of the bounding box projected to the plane. Initialize ray origin, direction, and attenuation with intersection point, outgoing direction, and inverse of the cross section area, respectively. 

Trace ray in loop until depth is reached (e.g., depth of 5), russian roulette breaks loop, or background is hit. If we hit the background and either the depth is > 0 or if we are in the bounding volume, record the incoming direction (negative of the exit direction). This requires transforming from cartesian to spherical coordinates. For every sample, multiply by 1/A, where A is the area of the incoming direction's bin. Accumulate samples in appropriate incoming direction bin for the given outgoing direction. Normalize all the incoming bins by the total number of samples sent for this outgoing direction (e.g., $4096^2$).

Results section

\subsection{Rendering performance}
\Steve{memory and time savings compare to GPU path tracer?}

\subsection{Prefiltering cost}
\Steve{Precomputation time? Training and data generation?}

\subsection{Notes and ideas}
\begin{itemize}
	\item{Recurrent net for encoding}
	\item{Add rendered image to test}
	\item{Phase function check if normalized based on outgoing direction}
	\item{Render higher spp GT}
	\item{Video moving camera smoothly through scene to see artifacts}
	\item{Instead of sampling 2D pdf is there a way to sample two 1D pdfs}
	\item{Talk about reciprocity}
\end{itemize}



